Resources: A Safe Language Abstraction for Money

Smart contracts are programs that implement potentially sophisticated transactions on modern blockchain platforms. In the rapidly evolving blockchain environment, smart contract programming languages must allow users to write expressive programs that manage and transfer assets, yet provide strong protection against sophisticated attacks. Addressing this need, we present flexible and reliable abstractions for programming with digital currency in the Move language [Blackshear et al. 2019]. Move uses novel linear [Girard 1987] resource types with semantics drawing on C++11 [Stroustrup 2013] and Rust [Matsakis and Klock 2014]: when a resource value is assigned to a new memory location, the location previously holding it must be invalidated. In addition, a resource type can only be created or destroyed by procedures inside its declaring module. We present an executable bytecode language with resources and prove that it enjoys resource safety, a conservation property for program values that is analogous to conservation of mass in the physical world.

==> fig-rules-proc.tex <==
\begin{figure*}
\begin{centerframe}


\semrule[\callRule]
  {
  }
  {\st{M,L,\stackht{r_{1}\cdots r_{n}}{R}}}
  {\to{\callCmd}{proc}}
  {\st{M,L,R}}\\
  \bigskip
  \yz{
    "TODO:
      this will require a fancier judgment form that includes the call stack
      Pop the $r_i$'s from the value stack, check that they match the
      signature of proc
      create a new stack frame for proc, load $r_{i}$'s into the L part of
      the new frame
    "
  }

\semrule[\returnRule]
  {
  }
  {\st{M,L,\stackht{r_{1}\cdots r_{n}}{R}}}
  {\returnCmd}
  {\st{M,L,R}}\\
  \yz{
    "TODO:
      this will require a fancier judgment form that includes the call stack
      Check that the $r_{i}$'s match the signature of the current proc
        Pop the call stack, leave value stack unchanged
        The caller will find the return value on the value stack
    "
  }
  \bigskip

\semrule[\abortRule]
  {
    c\in\dom{M}
  }
  {\st{M,L,\stackht{c}{R}}}
  {\abortCmd}
  {\execerror{\mread{M}{c}}}\\
  \yz{TODO: will need to add a new judgment form for this.
      Abort stops execution, returns the error code in M(c)
      and reverts all other state changes.
      Note: RejectUnless from the move paper has been replaced with Abort
  }
  \bigskip
\end{centerframe}
\caption{\label{fig:opsemCall}Operational Semantics of \move: Callstack related operations}
\end{figure*}


==> fig-rules-tree-2.tex <==
\begin{figure*}
\begin{centerframe}
\semrule[\loadtrueRule]
  {
  }
  {\st{M,L,R}}
  {\loadtrueCmd}
  {\st{{M},L,\stackht{\tv{\true}{\unres}}{R}}}\\
  \bigskip

\semrule[\addRule]
  {
    t_{1}=\tv{n_{1}}{\unres}\sep
    t_{2}=\tv{n_{2}}{\unres}\sep
    n_{1},n_{2}\text{ are integers }\sep
    n_{1} + n_{2} < 2^{64}
  }
  {\st{M,L,\stackht{t_{1}}{\stackht{t_{2}}{R}}}}
  {\addCmd}
  {\st{M,L,\stackht{{\tv{n_{1} + n_{2}}{\unres}}}{R}}}\\
  \bigskip

\semrule[\addErrRule]
  {
    t_{1}=\tv{n_{1}}{\unres}\sep
    t_{2}=\tv{n_{2}}{\unres}\sep
    n_{1},n_{2}\text{ are integers }\sep
    n_{1} + n_{2} \geq 2^{64}
  }
  {\st{M,L,\stackht{t_{1}}{\stackht{t_{2}}{R}}}}
  {\addCmd}
  {\execerror{Overflow}}\\
  \bigskip

\semrule[\notRule]
  {
    t=\tv{b}{\unres}\sep
    b\text{ is a Boolean }\sep
    t'=\tv{\neg b}{\unres}
  }
  {\st{M,L,\stackht{t}{R}}}
  {\notCmd}
  {\st{M,L,\stackht{t'}{R}}}\\
  \bigskip

  \caption{\label{fig:rules-tree-2}Operational Semantics of \move: Operations without accounts or callstack -- Part 2}
\end{centerframe}

\end{figure*}

